Intra- & Extra-Source Exemplar-Based Style Synthesis for Improved Domain Generalization

The generalization with respect to domain shifts, as they frequently appear in applications such as autonomous driving, is one of the remaining big challenges for deep learning models. Therefore, we propose an exemplar-based style synthesis pipeline to improve domain generalization in semantic segmentation. Our method is based on a novel masked noise encoder for StyleGAN2 inversion. The model learns to faithfully reconstruct the image, preserving its semantic layout through noise prediction. Using the proposed masked noise encoder to randomize style and content combinations in the training set, i.e., intra-source style augmentation (ISSA) effectively increases the diversity of training data and reduces spurious correlation. As a result, we achieve up to $12.4\%$ mIoU improvements on driving-scene semantic segmentation under different types of data shifts, i.e., changing geographic locations, adverse weather conditions, and day to night. ISSA is model-agnostic and straightforwardly applicable with CNNs and Transformers. It is also complementary to other domain generalization techniques, e.g., it improves the recent state-of-the-art solution RobustNet by $3\%$ mIoU in Cityscapes to Dark Z\"urich. In addition, we demonstrate the strong plug-n-play ability of the proposed style synthesis pipeline, which is readily usable for extra-source exemplars e.g., web-crawled images, without any retraining or fine-tuning. Moreover, we study a new use case to indicate neural network's generalization capability by building a stylized proxy validation set. This application has significant practical sense for selecting models to be deployed in the open-world environment. Our code is available at \url{https://github.com/boschresearch/ISSA}.

==> figs/landscape_sample_half.tex <==
\begin{figure*}[t]
    \begin{centering}
    \setlength{\tabcolsep}{0.0em}
    \renewcommand{\arraystretch}{0}
    \par\end{centering}
    \begin{centering}
    \hfill{}%
	\begin{tabular}{@{}c@{}c@{}c}
        \centering
		 Content & Style & Mixed  \tabularnewline
    \includegraphics[width=0.3\linewidth]{landscape_bochum_000000_027057_leftImg8bit.jpg} &
	{\footnotesize{}} \includegraphics[width=0.3\linewidth]{green_512x256.jpg} & {\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{bochum_000000_027057_green.png} 
	\tabularnewline
	
	\includegraphics[width=0.3\linewidth]{landscape_bochum_000000_000313_leftImg8bit.jpg} &
    {\footnotesize{}} \includegraphics[width=0.3\linewidth]{purple_512x256.jpg} & {\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{bochum_000000_000313_purple.png} 
	\tabularnewline
	
	\includegraphics[width=0.3\linewidth]{bear2_512x256.jpg} &
	{\footnotesize{}} \includegraphics[width=0.3\linewidth]{purple_512x256.jpg} & {\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{bear2_purple.png}
	\tabularnewline
		
	\includegraphics[width=0.3\linewidth]{driving_512x256.jpg} &
	{\footnotesize{}} \includegraphics[width=0.3\linewidth]{purple_512x256.jpg} & {\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{driving_purple.png}
	\tabularnewline
		
	\includegraphics[width=0.3\linewidth]{driving_blue_512x256.jpg} & {\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{driving_512x256.jpg} &
	{\footnotesize{}} 
	\includegraphics[width=0.3\linewidth]{driving_blue_driving.png}
	\tabularnewline
	
	\includegraphics[width=0.3\linewidth]{gray_512x256.jpg} &
	{\footnotesize{}} \includegraphics[width=0.3\linewidth]{green_512x256.jpg} & {\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{gray_green.png} 
	\tabularnewline
	
	\includegraphics[width=0.3\linewidth]{green_512x256.jpg} & {\footnotesize{}}
    \includegraphics[width=0.3\linewidth]{gray_512x256.jpg} &
	{\footnotesize{}}
	\includegraphics[width=0.3\linewidth]{green_gray.png} 
	\tabularnewline		
\end{tabular}
\hfill{}
\par\end{centering}
\caption{
Style-mixing using web-crawled images, where
the generator and encoder are only trained on Cityscapes. Except for the content images of the first 2 rows, all the others are web-crawled images.
\YL{to be updated!}
}
\label{fig:landscape-example}
\end{figure*}

==> tables/bn_iou.tex <==
\begin{table*}[t]
\begin{center}
{\small 
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{@{}l|ccccccccccccccccccc|c@{}}
Method & \rotatebox{90}{Road} & \rotatebox{90}{S.walk} & \rotatebox{90}{Build.} & \rotatebox{90}{Wall} & \rotatebox{90}{Fence} & \rotatebox{90}{Pole} & \rotatebox{90}{Tr.Light} & \rotatebox{90}{Sign} & \rotatebox{90}{Veget.} & \rotatebox{90}{Terrain} & \rotatebox{90}{Sky} & \rotatebox{90}{Person} & \rotatebox{90}{Rider} & \rotatebox{90}{Car} & \rotatebox{90}{Truck} & \rotatebox{90}{Bus} & \rotatebox{90}{Train} & \rotatebox{90}{M.bike} & \rotatebox{90}{Bike} & \rotatebox{90}{\textbf{mIoU}}\\
 \hline

Baseline &  74.4 &  33.9 &  45.0 &  12.7 &  18.1 &  14.1 & 30.2 & 26.8 & 55.5 & 20.9 & 54.3 & 17.9 & 10.8 & 59.5 & 27.6 & 25.8 & 31.4 & 17.1 & 10.3 &  30.9  \\

MixStyle\newcite{zhou2021mixstyle} &  75.6 &  32.0 &  57.0 &  21.8 &  21.2 &  17.7 & 44.6 & 32.9 & 65.6 & 25.4 & 65.1 & 25.7 & 10.6 & 55.9 & 32.4 & 37.8 & 43.4 & 18.1 & 19.7 &  37.0  \\
\textbf{{\ourstylebf} (Ours)} &  79.9 & 47.6 & 71.3 &  26.3 &  25.6 & 26.7 & 47.5 & 36.5 & 70.5 & 26.8 & 70.9 & 31.6 & 10.8 & 67.1 & 39.4 & 41.1 & 55.6 & 22.8 & 23.0 &  43.2 \\


\end{tabular}
}
\end{center}
\caption{Per-class IoU on ACDC. \YL{Not very helpful. Remove later!}}
\label{tab:bn_iou}
\end{table*}

==> tables/rebuttal_table_dg.tex <==
%%%%% Compare with UDA methods %%%%
\begin{table}[t]
\begin{center}
{\footnotesize  %\scriptsize %\footnotesize 
    {
    \begin{tabular}{l|c|ccc}
        Method & Network & Use Target & mIoU \\
    \midrule
        Baseline & \multirow{10}{*}{DeepLabv2
        %\deeplabvtwo
        } & \textbf{---} & 30.9 
        \\ \midrule
        BDL\scriptsize{\newcite{li2019bdl}} & & \cmark & 32.7 \\
        CRST \scriptsize{\newcite{zou2019confidence}}  &  & \cmark & 32.8 \\
        AdaptSegNet\scriptsize{\newcite{tsai2018AdaptSegNet}}  &  & \cmark & 33.4 \\
        SIM\scriptsize{\newcite{wang2020differential}}  &  & \cmark & 34.6 \\
        MRNet\scriptsize{\newcite{zheng2021rectifying}}  &   & \cmark & 36.1 \\
        ADVENT\scriptsize{\newcite{tsai2019advent}}  &  & \cmark & 37.7 \\
        CLAN\scriptsize{\newcite{luo2019clan}}  &   & \cmark & 39.0 \\
        FDA\scriptsize{\newcite{yang2020fda}}  &   & \cmark & 45.7 \\
        \ourstyle(Ours) &   & \xmark & 43.2 \\
        \midrule
        DAFormer\scriptsize{\newcite{hoyer2022daformer}} & DAFormer%\newcite{hoyer2022daformer}  
        & \cmark & 55.4\\
        \forRebuttal{
        PiPa\newcite{chen2022pipa}
        } 
        &  \forRebuttal{DAFormer} %\segformer  
        & \forRebuttal{\xmark} & \forRebuttal{44.6} \\
        \ourstyle(Ours) & SegFormer%\segformer  
        & \xmark & 52.5\\
    \end{tabular}
    }
}
\end{center}
\caption{Comparison with UDA methods on Cityscapes to ACDC generalization. Remarkably, our domain generalization method (without access to the target domain, neither images nor labels), is on-par or better than unsupervised domain adaptation (UDA) methods, which requires knowledge of the target domain during training. Results of UDA methods are from\acdc.}
\label{tab:rebuttal-uda-comparison}
\end{table}%$\rightarrow$
